Social Event Detection with Interaction Graph Modeling

This paper focuses on detecting social, physical-world events from photos posted on social media sites. The problem is important: cheap media capture devices have significantly increased the number of photos shared on these sites. The main contribution of this paper is to incorporate online social interaction features in the detection of physical events. We believe that online social interaction reflect important signals among the participants on the "social affinity" of two photos, thereby helping event detection. We compute social affinity via a random-walk on a social interaction graph to determine similarity between two photos on the graph. We train a support vector machine classifier to combine the social affinity between photos and photo-centric metadata including time, location, tags and description. Incremental clustering is then used to group photos to event clusters. We have very good results on two large scale real-world datasets: Upcoming and MediaEval. We show an improvement between 0.06-0.10 in F1 on these datasets.

==> abstract.tex <==
This paper focuses on detecting social, physical-world events from photos posted on social media sites. The problem is important: cheap media capture devices have significantly increased the number of photos shared on these sites. The main contribution of this paper is to incorporate online social interaction features in the detection of physical events. We believe that online social interaction reflect important signals 
%on part of 
among
the participants on the ``social affinity'' of two photos, thereby helping event detection. We compute social affinity via a random-walk on a social interaction graph to determine similarity between two photos on the graph. We train a support vector machine classifier to combine the social affinity between photos and photo-centric metadata including time, location, tags and description.
%to determine if a pair of photos belong to the same event. 
Incremental clustering is then used to group photos to event clusters. We have very good results on two large scale real-world datasets: Upcoming and MediaEval. We show an improvement between $0.06$--$0.10$ in F1 
%over the state of the art 
on these datasets. 

==> clustering.tex <==
\section{Event Detection}
\label{sec:event-det}

% % Incremental clustering algorithm
We learn first learn a photo similarity from multiple sources with Support Vector Machine (SVM) classifier, and then use an incremental clustering algorithm~\cite{Becker2010} to group photos into event clusters, 
%and use a SVM to combine the different sources of : social interactions and features. 
% The measure of similarity and the threshold to partition clusters are both important in determining high-quality clusters.

% How SVM is used and the 
The similarity measure between photos is critical in determine the performance of the event detection algorithm. Given there are multiple features available for each photo from Flickr, we choose an SVM classifier to combine these features together and produce a single value similarity measure $\theta(p_i,p_j)$ between a pair of photos $p_i, p_j$. 
%The input features for the SVM classifier are similarity values computed from all the selected features between the photo pairs.

On the training set, we first compile different features for classifier training. These include of similarity values from various photo and social features. While the similarity values of some photo features including time, photo-location are determined in a straightforward manner (Section~\ref{sec:photo}), the social similarity is computed via a random-walk algorithm on the social graph as described in Section~\ref{sec:social}. The SVM classifier is trained on pairs of photos that either belong to the same event (positive), or are from different events (negative). We randomly sample training pairs from the dataset, and the ratio of the negative to positive pairs is kept below 5 to to avoid skewing the prior.
%We generate the training pairs by randomly selecting photo pairs from the same event, and photo pairs from different event. The former is a positive example, while the latter pair constitutes a negative example. 

On the testing set, this SVM is applied on pairs of test photos, yielding a pair-wise similarity matrix. We then run a one-pass incremental clustering procedure to determine the event grouping. The algorithm incrementally assigns each photo $p_i$ into a cluster $C_k$ based on the similarity between this photo and existing clusters. To compute the photo--cluster similarity, we compute the average similarity between $p_i$ and each $p_j \in C_k$.
Specifically, given a similarity function $\theta$, a threshold $\mu$ and the photo stream $p_1, p_2, \dots, p_n$ We select the cluster that has the highest similarity value based on $\theta$ for each photo $p_i$ to be added. If no existing clusters whose similarity value to $p_i$ is greater than the threshold $\mu$, a new cluster is formed. We report results on a range of thresholds in the next section. 
%
%\begin{figure}
%    \includegraphics[width=0.5\textwidth]{incrementalcluster}
%    \caption{Incremental Clustering}
%    \label{figure:incrementalcluster}
%\end{figure}

% SVM model train, predict and how the features are used.
%The SVM classifier is first trained using the photo pairs generated from the development set before it is used to predict similarity value in the clustering framework. We generate the training pairs by randomly selecting photos from same event and using them as the positive data point, and photo pairs from different event as the negative data point. 

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% 
% % Conclude the similarity graph and social signal together boost the performance of the SED task and photo clustering in general.
% [rewrite, hari 7/29/12]

The goal of this paper was to detect social, physical-world events from photos posted on social media sites including Flickr. The main contribution of this paper was to incorporate social features in the detection of physical-events. We noted that prior work has  \textit{omitted social interaction as a feature} to detect events. We used a random-walk based approach to compute social affinity; this feature in addition to photo-centric metadata including time, location, tags and photo description to detect events.  We used an SVM classifier in conjunction with an incremental clustering method to detect events. We tested our algorithm on two large datasets---MediaEval and Upcoming---with significant improvement from non-social baseline.  Our goal was to demonstrate the utility of social interaction over baseline photo-features, despite that the final performance is not yet on par with the strongest in MediaEval 2011. We plan to improve our results by further tuning image- and text- based filtering methods coupled with social interaction. 


%We plan to further improve our performance to be on par with the top performer in MediaEval benchmark. This include incorporating image- and text- base filtering techniques to effectively eliminate noise from non-event photos.
%In both cases, our approach improves upon the state of the art by 10.2\% (Upcoming) and 5.9\% (MediaEval) respectively. We plan to extend our work by testing other social media datasets, including YouTube.

% Future work for graph similarity work.
%In the future, we plan to further validate the metric on event detection task with data-set from other more popular social media site e.g. YouTube. The richer user interactions on popular social media site may provide more insight on the impact of social signals of social event detection task. Further investigation on the importance of social signals can also be tested by adjusting the weight of edges in the graph i.e. construct multiple times of social favorite edges in similarity graph.

==> introduction.tex <==
\secmoveup
\section{Introduction}
\label{sec:intro}
\textmoveup

%[what is the problem, why is it important?]
The goal of this paper is to detect social, physical-world events from photos posted on social media sites including Flickr. The problem is important because the advent of cheap photo-capture devices, including mobile phones, has made it easy for people to capture and share media from physical events, such as concerts, festivals, and sports matches. This has resulted in a large number of photos being shared on social media sites. The large number of photos from such events makes it imperative that we are able to identify and organize event related photos.


%The problem is 
%% % Background and importance of social event detection
%Users uploaded over one million photos to Flickr and Facebook everyday. Mobile photos with high end camera enable users to take photos or videos during real world social event and upload the multimedia on the social network immediately. Thus increases the number of photos on the social media stream associated with real-world events. Being able to detect and organize these photos in the context of events benefits the media indexing and retrieval. We tackle the problem of social event detection by incorporating social interactions around multimedia on the social network.

% Formal definition of the SED task
%The task of social event detection~\cite{SED2011}(SED) requires system to identify photo clusters from a collection of photos where each cluster contains and only contains all the photos to represent the event. After the photo clusters has been identified, a retrieval method can be developed to answer queries for specific type of event. In this paper, we focus on clustering step and develop a new similarity metric for the clustering framework using random walk with restart on photo graphs.


%[who else has worked on this?]

Event detection on social media platforms has attracted considerable recent interest. 
Firan et al.~\cite{Firan2010} solves event detection as a supervised classification problem, where classifiers are built from the metadata of each event. 
Becker et. al.~\cite{Becker2010} poses this as an unsupervised clustering problem on social photo streams. This approach exploits a number of features including time, location and textual information. 
%first define similarity functions for the each individual feature and subsequently 
A classifier is trained to learn the similarity metric between photo pairs, and then photos are clustered into different event groups. 
Two other groups~\cite{Liu2011,Papadopoulos2011} uses visual analysis to find photos to illustrate and group events, community detection~\cite{Liu2011} is further introduced to improve performance.
%Their experiments show that the combination of time, 
%location and textual information produce the best result. 
% is also used to detect social events. 
In another recent work, Becker et al.~\cite{Becker2011twitterevent} designed a two-step approach to first cluster the input twitter stream and then perform event versus non-event classification on the clusters.
In all current approaches, photo content, tags, times and locations are used as the main features to cluster event photos. We note, however, that {\em social interactions} did not play a role in any of the prior approaches. 
%\textit{omitted social interaction as a feature} to detect events.
%\cite{Becker2012}


%
%%%%%%% Related work, RWR %%%%%%
%Random Walk with Restart has been previously used to compute the affinity of one node respect to another node within a graph. ~\cite{Pan2004} has used the RWR algorithm to successfully caption photos. The authors connect photos and keywords using their captioning edges. They apply RWR algorithm on the graph to compute the affinity of keywords for each photo. The photo captions are then obtained by selecting the keywords with the highest scores on the steady state probabilities.
%
%
%% Available data set and features to be used to detect events
%Specifically, we focus on the SED task on Flickr. There are several public available data sets~\cite{Becker:2010:LSM:1718487.1718524,SED2011} available to run experiments for this task. Topically, photos on Flickr have the following meta-data associated might help the task of SED:
%\begin{itemize}\itemsep -2pt
%\label{list:features}
%\item{\textbf{Time}: The taken time of the photo in ISO format according to the camera setting i.e. ``YYYY-MM-DD HH:MM:SS''. Available for all photos.}
%\item{\textbf{Location}: The location coordinates(latitude and longitude) of the photo indicate where the photo was taken. This partially available feature may be added by user manually or recorded by the camera.}
%\item{\textbf{Tag}: Short single word terms to label the photo, created by the owner or other people in the social network.}
%\item{\textbf{Text}: The title and descriptions of the photo entered by the owner.}
%%\item{Social: User can interact with each other by commenting or favoring other users' photos of their interests.}
%\end{itemize}
%
%% Previous approaches for SED. Our approaches for the SED task and contributions.
%Clustering algorithms including similarity learning~\cite{Becker:2010:LSM:1718487.1718524} and community detection~\cite{Papadopoulos:2011:CLE:1957374.1957482} are proposed to detect social events from collection of photos on Flickr using the above features. The effectiveness of the similarity metric directly influences the performance of clustering algorithms. In both approaches, tags along with times and locations are used as the main features to cluster event photos. One of the special feature for photos on social media networks, however, is omitted by all of the previous researches: social interactions on the photos among different users.

%[what have we done?]
The main contribution of this paper is to incorporate social features in the detection of physical-events. Real-world events are intrinsically social---they bring people together to participate in a shared experience. Therefore, it is natural to expect that co-participation in the physical event will motivate people who attended the event to interact online with shared media associated with that event. We argue that the social interaction reflect important and explicit signals on part of the participants on the ``social affinity'' of two photos, thereby helping in event detection. The social affinity between photos, in addition to photo metadata including time, location, tags and description are used to detect events. 

To compute social affinity between two photos, we proceed as follows. First we construct a directed, social interaction graph based on the relationship amongst users, tags and photos. Then, we use a random-walk model to determine similarity between two photos on the graph. This formulation appears naturally when we consider how users interact around shared photos with a social media site
%, including Flickr, where users share photos
. Then, we train a SVM on features from the social interaction graph and base photo features that have been shown to work well on event detection~\cite{Becker2010}. We shall use an incremental clustering algorithm on the photos to find event clusters. We tested our algorithm on two large datasets---MediaEval and Upcoming---with very good results. In both cases, our approach improves upon the state of the art by 0.102 (Upcoming) and 0.059 (MediaEval) respectively. 
%
%We argue that the social interactions on multimedia helps to task of SED. And further more, we propose a novel way to compute photo similarity on multimedia social network by taking advantages of these social signals and social graphs on multimedia social networks. In summary, the paper has following contributions:
%
%\begin{itemize}\itemsep -2pt
%\item{We test the impact of social interactions and social graph in the context of social event detection on multimedia social network.}
%\item{We develop a novel social and tag graph around the photos to measure the similarity between photos on Flickr.}
%\item{We test the algorithm on two public available data set to validate the performance of the similarity metric.}
%\end{itemize}

%[TOC] % Paper organization

The rest of the paper is organized as follows. In the next section, we introduce the idea of social affinity. Then, in Section~\ref{sec:photo}, we discuss the photo-features used as a baseline method for social event detection. In Section~\ref{sec:event-det}, we present our incremental clustering algorithm to detect events. In Section~\ref{sec:experiments}, we present our experimental results. Finally, we conclude with our summary and conclusions.

